On the Quantum Performance Evaluation of Two Distributed Quantum Architectures

Distributed quantum applications impose requirements on the quality of the quantum states that they consume. When analyzing architecture implementations of quantum hardware, characterizing this quality forms an important factor in understanding their performance. Fundamental characteristics of quantum hardware lead to inherent tradeoffs between the quality of states and traditional performance metrics such as throughput. Furthermore, any real-world implementation of quantum hardware exhibits time-dependent noise that degrades the quality of quantum states over time. Here, we study the performance of two possible architectures for interfacing a quantum processor with a quantum network. The first corresponds to the current experimental state of the art in which the same device functions both as a processor and a network device. The second corresponds to a future architecture that separates these two functions over two distinct devices. We model these architectures as Markov chains and compare their quality of executing quantum operations and producing entangled quantum states as functions of their memory lifetimes, as well as the time that it takes to perform various operations within each architecture. As an illustrative example, we apply our analysis to architectures based on Nitrogen-Vacancy centers in diamond, where we find that for present-day device parameters one architecture is more suited to computation-heavy applications, and the other for network-heavy ones. Besides the detailed study of these architectures, a novel contribution of our work are several formulas that connect an understanding of waiting time distributions to the decay of quantum quality over time for the most common noise models employed in quantum technologies. This provides a valuable new tool for performance evaluation experts, and its applications extend beyond the two architectures studied in this work.

==> SimNumerObs_old.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = manuscript.tex
\begin{figure}[t]
\centering
\subfloat[$\mu_e=10$, $\lambda_e=1$]{\includegraphics[width=0.4\textwidth]{Sims/comp_plots1/gate_mue_10_le_1}}\qquad\qquad
\subfloat[$\mu_e=500$, $\lambda_e=50$]{\includegraphics[width=0.4\textwidth]{Sims/comp_plots1/gate_mue_500_le_50}}
\caption{Average fidelity differences for two sets of entanglement request arrival rates and entanglement generation rates. Here, $T_1^{(1)}=T_1^{(2)}=0.00286$s and $T_2^{(1)}=T_2^{(2)}=0.001$s; $\mu_m^{(1)}=1667$Hz for all SD simulations. For all experiments, $\lambda_c = 150$ and $\lambda_m = 1000$.}
\label{fig:sim_comp_fidelity_low_T1T2}
\end{figure}
\begin{figure}[t]
\centering
\subfloat[$\mu_e=10$, $\lambda_e=1$]{\includegraphics[width=0.4\textwidth]{Sims/comp_plots11/mue_10_le_1_lambda_c_150_lambda_m_1000_new}}\qquad\qquad
\subfloat[$\mu_e=500$, $\lambda_e=50$]{\includegraphics[width=0.4\textwidth]{Sims/comp_plots11/mue_500_le_50_lambda_c_150_lambda_m_1000_new}}
\caption{Average fidelity differences for two sets of entanglement request arrival rates and entanglement generation rates -- $(c)$, $(d)$. Here, $T_1^{(1)}=10$s, $T_2^{(1)}=0.01$s, $T_1^{(2)}=2$s, and $T_2^{(2)}=0.002$s; $\mu_m^{(1)}=1667$Hz for all SD simulations. For all experiments, $\lambda_c = 150$ and $\lambda_m = 1000$.}
\label{fig:sim_comp_fidelity_high_T1T2}
\end{figure}
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.47\textwidth}
\centering
\includegraphics[width=1.05\textwidth]{Sims/lambda_e_225_lambda_m_1000_mu_e_500}
\captionof{figure}{Differences in average gate fidelity for the SD and DD architectures. For the latter, $T_1^{(2)}$ and $T_2^{(2)}$ are fixed at 0.00286s and 0.001s, respectively, while the ratios of the $T_1$ and $T_2$ times are varied. Here, $\mu_c=\infty$, $\lambda_e=225$, $\mu_e=500$, $\mu_m^{(1)}=1667$Hz, $\mu_m^{(2)}=700$Hz, and $\lambda_m=1000$ to ensure stability.}
\label{fig:comp_fid_v_T1T2}
\end{minipage}\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\includegraphics[width=\textwidth]{Sims/arch1_postmove_lambdam}
\captionof{figure}{Post-move fidelity for the SD architecture, as a function of the moving request rate $\lambda_m$. The characteristic memory times are varied at a constant ratio $T_1^{(1)}:T_2^{(1)}$, with initial values (\ie, when the multiplier is set to one) of $0.00286$s and $0.001$s for $T_1^{(1)}$ and $T_2^{(1)}$, respectively.}
\label{fig:arch1_pm_fidelity_v_T1T2}
\end{minipage}
\end{figure}
\begin{figure}[t]
\centering
\subfloat[Pre- and post-move fidelities for the DD architecture.]{\includegraphics[width=0.45\textwidth]{Sims/arch2_prepost_T1_2s_le_1_lc_150_mue_10_mum_700_muc_100000}}
\qquad\quad
\subfloat[Post-move fidelities for the SD and DD architectures. ]{\includegraphics[width=0.45\textwidth]{Sims/arch1_vs_arch2_post_T1_2s_le_1_lc_150_mue_10__mum1_1667_mum2_700_muc_100000}}
\caption{Pre- and post-move fidelities for the DD architecture, $(a)$, and post-move fidelities for the two architectures, $(b)$. Here, $T_1^{(2)}=2$s, $\lambda_e=1$, $\mu_e=10$, $\lambda_c = 150$, $\mu_c=10^5$,  $\mu_m^{(1)}=1667$Hz, and $\mu_m^{(2)}=700$Hz.}
\label{fig:arch12_sim_pm_ent_fidelity}
\end{figure}
\begin{figure}[t]
\centering
\subfloat[$\mu_e = 10,~\lambda_e=1$]{\includegraphics[width=0.45\textwidth]{Sims/comp_plots11/PrePostFidelity_mue_10_lambdae_1_lambdac_150}}\qquad\quad
\subfloat[$\mu_e = 1000,~\lambda_e=100$]{\includegraphics[width=0.45\textwidth]{Sims/comp_plots11/PrePostFidelity_mue_1000_lambdae_100_lambdac_150}}
\caption{Pre-move and post-move fidelities for varying computational job processing rates in the SD architecture, as functions of the moving request arrival rate $\lambda_m$. Here, $T_1^{(1)}=10$s and $T_2^{(1)}=0.01$s; $\lambda_c=150$ and $\mu_m^{(1)}=1667$Hz for all SD simulations and we assume the qubits are initially in a perfect entangled state.}
\label{fig:sim_ent_fidelity_high_T1T2}
\end{figure}
Our goal in this section is to study the average gate and entanglement fidelities for the two architectures in a variety of settings in order to gain an understanding of regimes that are most suitable to each. We will also explore differences in manufacturing quality, and examine cases where it is preferable to use an SD design of better quality than a DD design with poorer quality. This question is especially relevant when cost-effectiveness is an important factor, as the DD design is expected to be the more expensive option (when comparing to an SD design of identical quality).

We implement and simulate our model for the SD and DD architectures using MATLAB.  Our analytical results apply to the case when the processing time of computation requests is negligible, thus simulating the case where $\mu_c < \infty$ provides additional insight when considering computation requests that may block other requests.  We additionally make use of NetSquid \cite{coopmans2020netsquid}, a discrete-event network simulator for quantum information, in order to validate our derivations for the average gate fidelity of computation requests and the entanglement fidelity of move requests. NetSquid provides a hardware-validated model of the NV in diamond platform which allows us to implement the SD and DD architectures in order to simulate losses in fidelity due to imperfect quantum memories and quantum gates.  To evaluate the gate and entanglement fidelity of our architectures, we use our MATLAB code to obtain the waiting time distribution for different parameters and then use NetSquid to simulate the storage of qubits according to the obtained waiting time distributions.

For the case of $\mu_c<\infty$, computational jobs may no longer be processed instantaneously (as in the $\mu_c=\infty$ case). Thus, we require an additional rule in handling multiple computational requests in the queue. Motivated by the fact that entanglement generation with remote nodes is the most time-consuming operation for our architectures, we endow state transfer (moving) jobs non-preemptive priority over computational jobs, \ie, when a moving job arrives while a computation is in progress, the former begins processing immediately after the completion of the computational request, even if other computational jobs were already in the queue prior to its arrival.

For the following discussion, all rates are in terms of ($\#$ arrivals)/sec and ($\#$ jobs processed)/sec, unless otherwise specified. In all simulations, each run lasts for $10^5$ s, and each data point is an average of five runs. We next motivate some of the parameter values used in the remainder of this section, many of which are inspired by the NV center in diamond platform. For state transfers within the SD architecture, we fix $\mu_m^{(1)}$ at $1667$Hz, since \cf Figure 4 in \cite{pompili2021realization}, a local swap to memory consumes $600\mu s$. State transfers within the DD architecture depend on the exact implementation of the transfer procedure across the inter-device interface. For the DD architecture, we often fix $\mu_m^{(2)}=700$Hz, as we expect the state transfer rate in this architecture to be between a third and a half of that of the SD architecture. Note that, according to \cite{pompili2021realization} and \cite{ruf2021quantum}, for the NV, this value is rather optimistic, since \eg, a Bell-state measurement -- an operation that is part of the state transfer gate sequence for the DD architecture --  alone consumes 1ms. Next, when exploring different values for the computation rate, we consider the variation in not only gate duration, but also the possibility of more time-consuming atomic gate sequences that must not be interrupted by any other operations; using \cite{linkLayerPaper} as a guide, we set $\mu_c$ to values in the range $[10^3,10^5]$. For $T_1$ and $T_2$ values we use \cite{linkLayerPaper} as a guide.
Finally, when choosing parameter values for the request arrival rates, we ensure that both the SD and DD systems are stable in the number of outstanding entanglement requests. 
\subsubsection*{Effects of Device Memory Lifetimes}
Recall from our analytical evaluation that the DD architecture achieves higher gate fidelity than the SD architecture when both devices have the same $T_1$ and $T_2$ parameters characterizing their memory lifetime.  Figure \ref{fig:sim_comp_fidelity_low_T1T2} shows the difference in average gate fidelity for the two architectures under two different regimes of processing and arrival rates for entanglement requests.  Although our analytical evaluation makes the assumption that computation requests take zero time (\ie, $\mu_c=\infty$), we see that reducing the processing rate of computation requests still provides the DD architecture with an advantage over the SD architecture. However, increasing the processing and arrival rates of entanglement requests in both architectures reduces the difference in average gate fidelity between them.  This suggests that average gate fidelity differences become less prominent as entanglement generation rates of the two architectures improve.

Fabrication of networked quantum hardware is a complex task and achieving comparable memory lifetimes between the SD and DD architectures may prove to be difficult.  Interfacing the two processors that make up the DD architecture may introduce additional sources of noise or complicate the process of properly shielding qubits in order to maintain the memory lifetimes observed in the SD architecture.  Assuming one could fabricate a DD architecture with near-term memory lifetimes of the SD architecture, Figure \ref{fig:comp_fid_v_T1T2} shows how much the memory lifetime of the SD architecture must improve to gain a higher average gate fidelity, in the case of $\mu_c=\infty$. 
To provide additional insight in the case where the memory lifetime of the DD architecture is lower, we assume that $T_1^{(1)} > T_1^{(2)}$ and $T_2^{(1)} > T_2^{(2)}$. Each data point in Figure \ref{fig:comp_fid_v_T1T2} represents the difference between the SD and DD average gate fidelities for given $T_{1/2}^{(1/2)}$ values, with positive values representing cases where the SD performs better than the DD architecture. Note that not all combinations of $T_1$ and $T_2$ values are possible, as per the usual requirement that $T_1> T_2$. From the figure, we observe that the $T_2$ time plays a significant role in improving gate fidelity: note in particular that for lower values of $T_2^{(1)}$, the SD architecture does not outperform the DD architecture, even for very high values of $T_1^{(1)}$.
\subsubsection*{Effects of Processing Rates}
Processing rates impact the amount of time needed to complete requests and consequently the waiting times of other requests.  Our analytical evaluation assumed that $\mu_c=\infty$ so that computational requests do not interfere with entanglement and moving requests.
We use the computational job processing rate, $\mu_c$, to capture the behavior of different applications, where smaller processing rates may correspond to computation requests performing a sequence of atomic gates or 
computation requiring ``implicit'' state transfers (see Appendix \ref{app:NVoverview}).
In Figures \ref{fig:sim_comp_fidelity_low_T1T2} and \ref{fig:sim_comp_fidelity_high_T1T2}, we see that average gate fidelity differences tend to prefer the SD architecture as computational processing rates decrease (to see how the individual average gate fidelities evolve, see Appendix \ref{app:indivFidelityPlots}). In the case that the DD architecture has a poorer memory lifetime, we see that reducing $\mu_c$ leads to a higher gate fidelity in the SD architecture.  We additionally observe that the entanglement fidelity for moving requests is affected more so when entanglement processing rates are low as seen in Figure \ref{fig:sim_ent_fidelity_high_T1T2}.  In the case of the DD architecture, the gate fidelity of computation requests increases as the processing rate of moving requests $\mu_m^{(2)}$ increases.  These observations suggest that the SD architecture is better suited for settings such as a distributed quantum computing cluster where high entanglement generation rates can be achieved and longer computations must be performed.  In contrast, the DD architecture benefits from a setting such as long-distance quantum communication, with lower entanglement generation rates and high computation processing rates.
\subsubsection*{Effects of Arrival Rates}
The computation, entanglement, and moving request arrival rates impact the number of jobs that are issued to the system and consequently the probability that jobs block one another when non-zero processing time is assumed.  Since no jobs can be processed in parallel on the SD architecture, this leads to an overall increase in waiting time for all requests.  In contrast, computation jobs in the DD architecture are only blocked by moving jobs, while entanglement jobs may be processed in parallel.
One key observation is that both the arrival rates of entanglement requests and moving requests impact the the gate fidelity of computation jobs on the DD architecture.  By increasing the arrival rate of entanglement requests, additional moving requests are submitted which leads to a decrease in the gate fidelity of computation requests (as evidenced by Figures \ref{fig:sep_sim_comp_fidelity_low_T1T2} and \ref{fig:sep_sim_comp_fidelity_high_T1T2} in Appendix \ref{app:indivFidelityPlots}).  In contrast, we observe an increase in the gate fidelity of the SD architecture here as the entanglement generation rate also increases, leading to a decrease in the amount of time that computation requests are blocked from processing.
The arrival rates additionally impact the pre- and post-move entanglement fidelity as visible in Figure \ref{fig:sim_ent_fidelity_high_T1T2}.  The moving request arrival rate can be seen as the system's responsiveness to newly established entanglement. From this we learn that the faster decisions for moving entanglement are made, the higher the resulting entanglement fidelity. Note from Figure \ref{fig:arch1_pm_fidelity_v_T1T2} that the required responsiveness depends on the $T_1$ and $T_2$ parameters and that the moving request arrival rate may be reduced if higher memory lifetimes are available.
\subsubsection*{Effects of Moving Entanglement}
Recall from Section \ref{sec:quantum_bg} that the SD and DD architectures process moving requests in different ways. The SD architecture performs a sequence of local gates whereas the DD architecture must execute a network operation to transfer entanglement from the networking to the computing device. We detail these processes for the NV example further in Appendix \ref{sec:nv_state_transfer}.  Since we assume that quantum gates in both architectures are imperfect, it is important to highlight the differences in entanglement fidelity once a moving request has been processed.

Figure \ref{fig:sim_ent_fidelity_high_T1T2} shows the reduction between the pre-move and post-move entanglement fidelity for the SD architecture. We see that the post-move fidelity approaches an asymptotic limit of $\approx 0.95$ as the pre-move fidelity approaches $1$. The post-move entanglement fidelity is limited due to the inherent noise of the quantum gate sequence used to process moving requests.
In contrast to the SD architecture, processing moving requests in the DD architecture requires entanglement between the communication and computation devices as well as a lengthier sequence of quantum gates. We find that the post-move entanglement fidelity in the DD architecture depends strongly on $T_2^{(2)}$ characterizing the memory lifetime due to the amount of time entanglement needs to be held in the computing device while teleportation is performed on the networking device.  We also observe that increasing $T_2^{(2)}$ leads to the post-move fidelity approaching an asymptotic limit of $\approx 0.86$ which corresponds to inherent fidelity reduction due to the quantum gates used to move entanglement. From this we believe that the DD architecture may be suitable for applications that observe lower fidelity requirements on entanglement as the inherent reduction in fidelity restricts this architecture from being useful to applications with higher fidelity requirements.
% EVALUATION QUESTIONS

% \subsection{How much better do memory lifetimes of the single-NV architecture need to be?}
% From our analytical evaluation we concluded that if the single-NV and double-NV have the same $T_1/T_2$ times characterizing their memory lifetime, then the double-NV architecture will always outperform the single-NV architecture in terms of computation request gate fidelity. One may then wonder how much better the memory of the single-NV architecture needs to be in order to achieve higher gate fidelity than the double-NV architecture. We find that the answer to this additionally depends on other parameters of our CTMC model.  In figure \ref{fig:comp_fid_v_T1T2}, we see that gaining an advantage of $0.01$ in terms of computational gate fidelity would potentially require increasing both the $T_1$ and $T_2$ times by a factor of $4$ each.   We also observe that improving the gate fidelity of the single-NV architecture strongly depends on improving its $T_2^{(1)}$ time as well. The required improvement in $T_2^{(1)}$ to match the computation request gate fidelity of the double-NV architecture reduces marginally as $T_1^{(1)}$ improves. Such improvements in memory lifetime may be prohibitively difficult to achieve, thus focusing on improving the memory lifetimes of the double-NV architecture may be a preferable approach to designing quantum hardware with higher performance.

% Our analytical observation is further supported by our simulations as shown in figure \ref{fig:sim_comp_fidelity_low_T1T2}. Consider figure \ref{fig:sim_comp_fidelity_high_T1T2} where the $T_1/T_2$ times of the double-NV architecture are a factor of ten worse than those of the single-NV architecture.  Here we observe that the performance difference between the two architectures depends on the processing rate of computation requests when fixing the arrival and processing rates of entanglement requests.  Lower $T_1/T_2$ times cause the gate fidelity of computation requests to be more sensitive to lower processing rates $\mu_c$, resulting in lower gate fidelity. We additionally see that increasing the entanglement request arrival rate and entanglement generation rate reduces the gate fidelity of the double-NV architecture even further, making it easier for the single-NV architecture to achieve higher gate fidelity.  This is because increasing the entanglement request arrival rate introduces additional moving requests which block computation requests from being executed in the double-NV architecture.

% \subsection{How fast does entanglement need to be generated?}
% As mentioned, the double-NV architecture always achieves higher computation request gate fidelity than the single-NV architecture when the $T_1/T_2$ times characterizing their memory lifetimes are the same. When the single-NV has a better memory lifetime, one than the double-NV architecture.  From figure \ref{fig:sim_comp_fidelity_low_T1T2} we observe that increasing the entanglement generation rate and entanglement request arrival rate reduces the difference in gate fidelity below $0.025$ even when computation requests have zero processing time and the two architectures have the same memory lifetimes. When the single-NV architecture has a higher memory lifetime, the minimum entanglement generation rate that allows achieving higher computation request gate fidelity becomes lower as visible in figure \ref{fig:sim_comp_fidelity_high_T1T2}. Here, we see that computation requests with longer processing times benefit more from the single-NV architecture even for lower entanglement generation rates.

% Having gate fidelity depend on entanglement generation further suggests that the single-NV and double-NV architectures may be suitable for different tasks.  In a distributed quantum computing cluster, where a larger processor is formed by connecting a set of smaller, networked quantum processors, entanglement generation rates may be relatively high, suggesting that using single-NV architecture devices could provide higher performance.  However, in the realm of long-distance applications, where lower entanglement generation rates are achieved, the double-NV architecture may achieve higher gate fidelity for computation requests depending on how much worse the memory lifetimes are.


% \subsection{How much faster does moving entanglement in double-NV need to be?}
% In figures \ref{fig:sim_comp_fidelity_low_T1T2} and \ref{fig:sim_comp_fidelity_high_T1T2} we consider the difference in gate fidelity between the two architectures as a function of how quickly entanglement may be stored in the double-NV architecture.  Here, we restrict our analysis to the regime where $\mu_m^{(2)} \ge \mu_e$ as $\mu_e$ depends on the distance over which entanglement is established and we expect that doing so between the NVs in the double-NV architecture would be faster than establishing entanglement with a separate quantum processor over larger distances.

% We observe a general trend that gate fidelity favors the double-NV architecture more as the rate of processing moving requests increases. For lower entanglement generation rates, we see from figure \ref{fig:sim_comp_fidelity_high_T1T2} that if the computation request processing rate is relatively high, then the double-NV architecture can outperform the single-NV architecture even for moving request processing rates that are an order of magnitude lower than that in the single-NV architecture.  An implementation of the double-NV architecture with low move request processing rate thus finds itself better suited for applications with low entanglement request arrival rate as it consequently reduces the number of moving requests that will block computation requests from being processed.

% \subsection{How quickly must movement of entanglement begin?}
% We now wish to turn our attention to the entanglement fidelity and consider how quickly the architectures must receive requests for moving entanglement in order to maintain high fidelity of the established state. The fidelity of entangled qubits delivered to applications depends on how quickly they are moved into memory, which in turn depends on how quickly a moving request will be issued once entanglement has been generated.  Using eq. \ref{eq:arch1_pm_fidelity} we construct figure \ref{fig:pm_fidelity_v_T1T2} to show the trade-off between memory lifetime and the moving request arrival rate. From this we learn that an alternative approach to increasing entanglement fidelity may be to focus on designing low-latency control for a quantum processor rather than focusing on improving the quality of the memory.

% Our simulation results in figure \ref{fig:sim_ent_fidelity_high_T1T2} show that increasing the moving request arrival rate results in a higher entanglement fidelity both after executing the move and immediately before it. This is because increasing the moving request arrival rate reduces the time generated entanglement must wait to be moved into memory.  When increasing the entanglement request arrival rate $\lambda_e$ and entanglement processing rate $\mu_e$, we see that the requirement for $\lambda_m$ to achieve pre-move and post-move fidelity greater than $0.9$ relaxes for $\mu_c=1000$. In the single-NV architecture, the rate of entanglement request arrival and entanglement processing influences the number of outstanding computation requests that queue while entanglement is generated.  By generating entanglement more quickly, less computation requests will be submitted while entanglement is generated which reduces the likelihood that a computation job is in-progress once a moving request arrives to store the entanglement. 

% PLOT OBSERVATIONS

% Figure \ref{fig:sim_comp_fidelity_low_T1T2} shows the performance difference between the single-NV and double-NV architectures in terms of average gate fidelity for computational jobs when both architectures have the same $T_1$ and $T_2$ times characterizing their memories. From figures \ref{fig:sim_comp_fidelity_low_T1T2}a we see that increasing $\mu_e$ and $\lambda_e$ for the single-NV architecture results in a higher gate fidelity. Recall that only one job may be actively processed at any time in the single-NV architecture, here we see that increasing the rate of entanglement job processing reduces the amount of time that computational jobs must wait before being processed and consequently increases their associated gate fidelity.

% In the double-NV architecture, however, entanglement jobs may be processed in parallel with computational jobs, but moving entanglement from the communication NV to the computing NV blocks computation jobs from being processed. From \ref{fig:sim_comp_fidelity_low_T1T2}b we see that increasing $\mu_m^{(2)}$ causes the gate fidelity of computation jobs to increase even as $\mu_e$ and $\lambda_e$ increase. Increasing $\mu_m^{(2)}$ results in shorter processing time for move requests which reduces the waiting time of computation jobs that need to be put on-hold during moving jobs.

% Figures \ref{fig:sim_comp_fidelity_low_T1T2}c and \ref{fig:sim_comp_fidelity_low_T1T2}d show the relative difference in gate fidelity of computation jobs as a function of the rate of processing moving requests on the double-NV architecture.  Here, the $T_1$ and $T_2$ times characterizing the memory lifetime of the single-NV and double-NV architectures are the same and we see that the double-NV architecture outperforms the single-NV architecture when varying the rate of processing computation jobs.  \ms{How can we explain the decrease in difference as $\mu_c$ decreases?}

% Figure \ref{fig:sim_comp_fidelity_high_T1T2} expands upon the results in figure \ref{fig:sim_comp_fidelity_high_T1T2} by showing the performance difference of computational jobs when the $T_1/T_2$ times of the double-NV architecture are five times lower than that of the single-NV architecture.  Similarly to figure \ref{fig:sim_comp_fidelity_low_T1T2}a, figure \ref{fig:sim_comp_fidelity_high_T1T2}a shows the effect of increasing $\lambda_e$ and $\mu_e$ on the average gate fidelity of computation jobs.

% We learn from figure \ref{fig:sim_comp_fidelity_high_T1T2}b that when the rate of processing moving jobs on the double-NV architecture is fixed while $\lambda_e$ and $\mu_e$ are increased, that the gate fidelity of computation jobs decreases. The reason for this is that increasing the rate of arrival of entanglement jobs results in more moving jobs being submitted to the system, which introduces additional blocking of computation jobs that are executed on the computation NV. This shows that the double-NV architecture must have a sufficiently high rate of processing moving jobs if it is to accommodate larger amounts of entanglement jobs while maintaining high gate fidelity of computation jobs.

% In contrast to figures \ref{fig:sim_comp_fidelity_low_T1T2}c and \ref{fig:sim_comp_fidelity_low_T1T2}d, figures \ref{fig:sim_comp_fidelity_high_T1T2}c and \ref{fig:sim_comp_fidelity_high_T1T2}d illustrate that the single-NV architecture is preferable when it has higher memory lifetimes than the double-NV architecture. As $\lambda_e$ and $\mu_e$ increase, larger amounts of moving jobs are introduced into the system causing computation jobs to wait longer. The poorer memory lifetime of the double-NV architecture then cause a larger reduction in the gate fidelity of computation jobs than experienced on the single-NV architecture with higher memory lifetime.

% Figure \ref{fig:sim_ent_fidelity_high_T1T2} shows the fidelity of entanglement from entanglement jobs before and after the execution of the moving job. We observe that increasing $\lambda_m$ results in a higher entanglement fidelity before moving the entanglement as it reduces the amount of time entanglement waits for a moving job. This consequently results in a higher entanglement fidelity after the moving job as well.

% From these figures we also learn that increasing the rate of processing computation jobs additionally results in higher entanglement fidelity. Reducing the amount of time it takes to process computation jobs reduces the waiting time of moving jobs should one arrive while a computation job is being processed, resulting in a higher entanglement fidelity.
